Efficient Byzantine Fault Tolerance using Trusted Execution Environment: Preventing Equivocation is only the Beginning

With the rapid development of blockchain, Byzantine fault-tolerant protocols have attracted revived interest recently. To overcome the theoretical bounds of Byzantine fault tolerance, many protocols attempt to use Trusted Execution Environment (TEE) to prevent equivocation and improve performance and scalability. However, due to the broken quorum intersection assumption caused by the reduction of the replica number, the improvement is mostly at the cost of increased communication complexity which prevents existing TEE-based protocols to be applied to large-scale blockchain systems. In this paper, we propose TBFT, an efficient Byzantine fault-tolerant protocol in the partial synchrony setting, which has O(n) message complexity in both normal-case and view-change. Compared to previous protocols, TBFT uses TEE-assisted primitives to limit more types of malicious behaviors of replicas rather than preventing equivocation only, thereby reducing the latency and communication complexity of clients and replicas. Besides, we also introduce lightweight cryptographic primitives including a novel leader election mechanism and an efficient voting message aggregation mechanism for better security and performance. We evaluate TBFT via systematic analysis and experiments, and the results show that TBFT has better performance and scalability compared to other protocols.

==> CFT.tex <==
In this section, we discuss new security issues faced by TEE-based BFT by revisiting popular CFT protocols. We choose the most popular TEE, \ie, Intel SGX, and Raft\cite{184040}, one of the most popular and understandable CFT protocols to demonstrate those issues and propose four principles, \ie, one proposal, one vote, restricted commit, and restricted log generation to solve them. 
\subsection{TEE with Byzantine Host}
The core difference between TEE-based BFT and CFT is that the host in TEE-based BFT may be byzantine. As we mentioned before, a malicious host can arbitrarily manipulate its local TEE. It can arbitrarily manipulate TEE scheduling and I/O. It can drop, replay, delay, reorder, modify the I/O messages of TEE arbitrarily, schedule TEE in any sequence, or even terminate TEE at any time. 
Through these malicious behaviors, the byzantine host may deceive other replicas to break the safety and liveness of the system. The following four principles use TEE to tolerate those behaviors and bridge the gap between TEE-based BFT and Raft. 

\subsection{One Proposal}
In Raft, at the beginning of a log replication, the leader will choose a client request and replicate it to other replicas as an entry. Once the entry has been safely replicated to majority replicas, the leader will tell other replicas to commit this entry. However, in BFT, a malicious leader may propose different proposals to different subsets of replicas, \ie, equivocating. As we mentioned in section \ref{sec:background}, this will lead to inconsistent states among replicas. 

Similar to previous work, we use trusted monotonic counters to prevent leader equivocation. As shown in Algorithm \ref{alg:1}, we provide TEE primitives as a trusted monotonic counter. The leader needs to call CREATE\_COUNTER to assign a (c,v) for each proposal while other replicas will keep track of the leader's (c,v). Upon calling CREATE\_COUNTER, TEE will increase its local monotonic counter. Hence, there will never be two different proposals with the same(c,v) value so that the equivocation can be prevented. In this paper, we called this One Proposal Principle, \ie, the leader can not propose multiple proposals in the same round. 
\subsection{One Vote}
In Raft, if an entry has been safely replicated to majority replicas, it is committed. Raft guarantees that committed entries are durable and will be executed by all of the available state machines eventually. However, byzantine hosts can use this to break safety. For instance, assume a network partition occurs and all f+1 non-faulty replicas are split into two subsets. The non-faulty replicas in the different subsets cannot communicate with each other while all f byzantine replicas can still communicate with all replicas. Due to the network partition, there may be multiple leaders, \ie, stale leaders, and the current leader, proposing different proposals at the same time. In Raft, a replica will only accept one proposal so that only one proposal will be replicated to majority replicas successfully and get committed. However, in TEE-based BFT, a byzantine replica may vote for multiple proposals. Then more than one proposal will collect f+1 votes and get committed. This will lead to inconsistent states among replicas. 

Hence, TEE-based BFT should guarantee that a replica can not vote for more than one conflicting proposals. We called it One Vote Principle. The corresponding primitives are shown in Algorithm \ref{alg:1}.  Upon calling VERIFY\_COUNTER, TEE will check the (c,v) of the proposal. If the (c,v) is matched with its local (c,v), TEE will increase its local monotonic counter. Otherwise, it will reject to vote for it. By doing so, we solve the problem above. 

\subsection{Restricted Commit}
Raft has a strong leader model. The leader is responsible for notifying other replicas to commit proposals. However, in TEE-based BFT, a byzantine host may lie that a proposal has been safely replicated to majority replicas to let non-faulty replicas commit a proposal. 

Hence, the leader should prove that a proposal has been safely replicated to majority replicas. Generally, this proof is called Quorum Cert(QC) in BFT. Upon receiving a proposal, each replica will send a vote to the leader. Upon collecting at least f+1 votes, the leader can generate a QC and send it to all replicas as proof of commit. As suggested in \cite{8419336}, we use light-weight TEE-assisted secret-sharing to replace multi-signature. The corresponding primitives are described in Algorithm \ref{alg:1}.

\subsection {Restricted Log Generation}
In Raft, each replica needs to be honest about the entry they have received. It is essential when a new leader election happens. However, this is not trivial in TEE-based BFT. TEE only has limited resources, \eg, Intel SGX only has 128MB memory currently. Hence, TEE has to store message logs via untrusted hosts. A byzantine host may modify those message logs, \eg, drop message logs arbitrarily. Besides, it can generate a stale message log previously and replay this message log. In Algorithm \ref{alg:1}, we design a TEE-based mechanism to solve this problem. With this mechanism, we restrict the log generation and guarantee that all replicas have to be honest about the entries they voted for, \ie, if replica $S_i$ voted for proposal p in view v, then it can only generate a valid message log L that contains p (or do nothing). For simplicity, we leave the proof in Section \ref{sec:proof}. 
\begin{tiny}
\begin{algorithm}
	\caption{TEE-assisted Primitives}
	\begin{algorithmic}[0]
		\State $c, v$ \Comment{$c$ is the current value of $S_i$'s monotonic counter, v is the current view(maintained by all replicas)}		
	\State $c', v'$ \Comment{value of the last validated counter(c,v) }
	%\State $L$ \Comment{all valid messages received by each replica in the current view (maintained by all replicas)}
	\State $\{S_i,pk_i\}$ \Comment{all replicas and their public keys}
	\State $\{S_i, k_i\}$ \Comment{all replicas and their symmetric keys}\newline
	%\State $k_i $ \Comment{current view key(maintained by all repicas)}\newline
	
	
	%生成secret的函数
	\Function{generate\_secret}{$c''$,$v''$} \Comment{for $S_p$}
	\State s=\textbf{rand}( )
	\State $h_{c''}$=\textbf{Hash}(s)
	\State $\{s_i\}_i \leftarrow s $ \Comment{Shamir-Secret-Sharing}
	\State $\xi_{c''}^i=E(k_i,<s_{c''}^i,(c'',v''),h_{c''}>)$
	\State $<h_{c''},(c'',v'')>_{\sigma_p}$=$Sign(<h_{c''},(c'',v'')>)$
	\State \textbf{Return} $\{<h_{c''},(c'',v'')>_{\sigma_p}, \xi_{c''}^i\}_i$
	\EndFunction 
	
	%请求counter的函数
	\Function{create\_counter}{x} \Comment{for $S_p$}
	\State $<x,(c,v)>_{\sigma_p} = Sign(<x,(c,v)>_{\sigma_p} )$
	\State $c=c+1$
	\State \textbf{Return} $<x,(c,v)>_{\sigma_p} $
	\EndFunction
	
	%验证并销毁counter的函数
	\Function{verify\_counter}{$<x,(c_p,v_p)>_{\sigma_p}, \xi_{c''}^i$} 
	\Comment{for all replicas}
	
	\If {Vrfy($<x,(c_p,v_p)>_{\sigma_p}$)==false}
	\State \textbf{Return} REQ-VIEW-CHANGE::Invalid\_Message
	\Else
	\State  $<s_{c''}^i, (c'',v''), h_{c''}>$ = D($\xi_{c''}^i$) 
	\EndIf
	\If {$(c_p,v_p)!=(c'',v'')$ \textbf{or} $c!=c_p$ \textbf{or} $v!=v_p$ }
	\State \textbf{Return} REQ-VIEW-CHANGE::Invalid\_Counter
	\EndIf
	\If{$(v'==v_p$ \textbf{and} $c'+1==c_p)$ \textbf{or} $(v'<v$ \textbf{and} $c_p==0)$}
	\State $c'=c_p; v'=v_p; $
	\State $c=c+1$
	\EndIf
	\EndFunction
		%收集并合并message log的函数
		\Function{merge\_message\_logs}{$\{\langle L,\langle H(L),(c_i,v_i)\rangle _{\sigma_i}\}_i $} \Comment {for next primary replica $S_{p'}$ }
		\For {each \textbf{L} in $\{\langle L,\langle H(L),(c_i,v_i)\rangle _{\sigma_i}\}_i $}
		\If {vrfy(L)==true}
		\State O.merge(L)
		\EndIf
		\EndFor
		\State update\_counter(O) \Comment {update c, v, c', v' according to O}
		\State $\langle H(O),(c,v)\rangle \sigma_{p'}$=TEE.create\_counter(H(O))
		\State \textbf{Return} $\langle H(O),(c,v)\rangle \sigma_{p'}$
		\EndFunction
		\Function{get\_message\_logs}{L} \Comment{for all replicas}
		\If {vrfy(L)==true}
		\State $\langle H(L),(c,v)\rangle _{\sigma_i}$=TEE.create\_counter(H(L))
		\State \textbf{Return} $\langle H(L),(c,v)\rangle _{\sigma_i}$
		\Else 
		\State \textbf{Return} ERROR::Invalid\_messgae\_log
		\EndIf
		\EndFunction
		\Function{update\_view}{$\langle O,\langle H(O),(c_{p'},v_{p'})\rangle \sigma_{p'},$ $e_i\rangle $} \Comment {for all replicas}
		\If {Vrfy($\langle O,\langle (H(O),(c_{p'},v_{p'})\rangle \sigma_{p'}\rangle $)==true}
		\State update\_counter(O) \Comment {update c, v, c', v' according to O}
		\EndIf
		%				\State \textbf{Return} REQ-VIEW-CHANGE::Invalid\_Signature
		%			\ElsIf { c!=$c_{latest}+1$ }
		%\State \textbf{Return} REQ-VIEW-CHANGE::Invalid\_Counter
		%\EndIf
		\EndFunction
	\end{algorithmic}
	\label{alg:1}
\end{algorithm}
\end{tiny}


==> Chained-TBFT.tex <==

In basic \prot protocol, each request requires two phases (PREPARE and COMMIT) to get processed. In each phase, the primary replica needs to generate a secret, collect f+1 votes from all replicas and generate a QC which has a big impact on performance. However, in basic \prot, one valid QC is used for only one phase which is quite inefficient. 
%i.e., only represents that the current proposal is acceptted by at least f+1 replicas. 
In chained \prot protocol, we make full use of QCs by pipelining QCs. e.g., the Commit QC of the current request also serves as the Execute QC of the previous request.

Chained \prot and Basic \prot are mostly the same, but there are still some key differences. As Fig \ref{sec:acknowledgement} shown, in Chained \prot, each replica needs to maintain a QC-Chain. Each proposal p needs to points to a previous proposal p'(p and p' may not have consecutive (c,v) values due to potential view-change). If p' is not the latest voted proposal of $S_i$, then $S_i$ will not vote for p.


\begin{figure}
	\centering
	\includegraphics[width=.5\textwidth]{./graph/pipeline.png} %1.png是图片文件的相对路径
	\caption{Chained \prot } %caption是图片的标题
	\label{img:pipeline}
\end{figure}

In view-change case of chained \prot Protocol, after receiving f+1 REQ-VIEW-CHANGE,  the next primary replica $S_{p'}$ will generate a message log O and send it to all replicas. After validating O, $S_i$ will vote for it. Upon receiving at least f+1 votes, $S_{p'}$ can generate a NEW-VIEW-QC and send it to all replicas. The NEW-VIEW-QC will also influence other rounds, i.e., the NEW-VIEW-QC also serves as the Commit-QC of the last request in the previous view. 

Algorithm 5
\begin{algorithm}
	\caption{Normal-case Operation in Chained \prot}
	\begin{algorithmic}[0]
		\Event{reception of f+1 $<Generic-Vote, s_c^i>$ at $S_p$}
		\State $s_c \leftarrow  \{s_c^i\}_i$ \Comment {Shamir Secret Sharing, $s_c$ is the Generic-QC}
		\State $res' \leftarrow execute \quad M'$
		\State M=get\_new\_request( );
		\State $x\leftarrow H(M|res'|M')$
		\State $<x,(c+1,v)>_{\sigma_p}$=TEE.request\_counter(x)
		\State $\{<h_{c+1},(c+1,v)>_{\sigma_p}, \xi_{c+1}^i\}_i$=TEE.generate\_secret(c+1,v)
		\State send $<Generic-Proposal,s_c,M,res',<x,(c+1,v)>_{\sigma_p},<h_{c+1},(c+1,v)>_{\sigma_p}, \xi_{c+1}^i>_i $ to each replica $S_i$
		\State send $<DECIDE, res, <H(M''|res''|M'),(c,v)>_{\sigma_p},<h_{c},(c,v)>_{\sigma_p}, s_{c}, <H(M'''|res'''|M''), (c',v')>_{\sigma_p},<h_{c'},(c',v')>_{\sigma_p},s_{c'}>$ to client \Comment{proof-of-execute of M''}
		\EndEvent\newline
		
		\Event{reception of $<Generic-Proposal,s_c,M,res',<x,(c+1,v)>_{\sigma_p},<h_{c+1},(c+1,v)>_{\sigma_p}, \xi_{c+1}^i>_i $at $S_i$}
		\If {H($s_c$) != $h_c$ \textbf{or} execute op' != res'} 
		\State Request for View-Change
		\Else
		\State $<s_{c+1}^i, h_{c+1}>$=TEE.verify\_and\_increase\_counter($<x, (c+1,v)>_{\sigma_p},\xi_{c+1}^i$)
		\State send $<Generic-Vote, s_{c+1}^i>$ to $S_p$ 
		\EndIf
		\EndEvent\newline
	\end{algorithmic}
\end{algorithm}

==> VRF.tex <==

In this section, we discuss the leader election mechanism in \prot. In traditional BFT protocols, the result of leader election is predictable, e.g., in Hotstuff\cite{10.1145/3293611.3331591}, each replica has a number, and the primary replica for view v is v\%n, where n is the number of replicas. However, a predictable leader election mechanism leads to many serious problems, e.g., an adversary may launch a DoS(Denial of Service) attack against the primary replica. By predicting the next primary replica and launching DoS attacks against it successively, the attacker can bring the system down for a long time. 

To avoid such attacks, an unpredictable leader election mechanism is needed. However, this is not trivial. 
%because liveness should always be guaranteed while making the leader election unpredictable.
%TODO: 添加hotstuff引用
Every replica should have a consensus on the next primary replica while the mechanism must be distributed(or a single-point failure may bring the system down). Distributed Verifiable Random Function(DVRF)\cite{galindo2020fully} can solve this problem. However, traditional DVRF solutions\cite{dodis2003efficient}\cite{kuchta2013unique}\cite{galindo2020fully}  rely on complex cryptographic methods, e.g. threshold
BLS signatures\cite{boneh2004short} or publicly verifiable
secret sharing(PVSS)\cite{stadler1996publicly}. To generate one random number, replicas may need to run multi-round protocols or do expensive computation which means large communication and computation overhead.
%TODO:详细叙述传统VRF的弊端

Utilizing TEE, we introduce a novel and efficient solution for unpredictable and verifiable leader election. During initialization, TEEs will share a random seed via secret sharing. All TEEs uses the same random function(Remote Attestation guarantees verifiability). So with the same input sequence, they will generate the same random number. 
%Recall that BFT will guarantee that all replicas execute requests in the same order so that all non-faulty  replicas will reach a consensus about the random number. 
In detail, replicas will use $H(s)$ to generate a random number r and regard r\%n as the next primary replica where $H(s)$ is the hash of the last valid secret in v' and v' is the previous view of v. Recall that before changing to the next view v, all replicas will process all proposals in v' in the same order so that every replica will have a consensus on $H(s)$. Note that each secret is a random number generated in TEE, so its value is unpredictable. 

By doing so, we delay the announcement of election results, i.e., only after view v-1 finishes, faulty replicas can know the primary replica of view v+1. It will effectively limit the window of time for attackers to launch attacks, e.g., DoS attacks against the primary replica. Besides, this solution only has $O(1)$ communication and computation complexity which is much more efficient than other solutions. 

==> keywords.tex <==
State Machine Replication, Byzantine Fault Tolerance, Trusted Execution Environment


==> resultfigure.tex <==
\begin{figure*}
	\centering
	\begin{subfigure}{0.42\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Tps_Txn_bar.pdf}
		\caption{Average Tps with varying number of transactions}
		\label{fig:tpstxn}
	\end{subfigure}
	\quad
	\begin{subfigure}{0.42\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Latency_Txn.pdf}
		\caption{Execution Time with varying number of transactions}
		\label{fig:LatencyTxn}
	\quad
	\end{subfigure}
	\begin{subfigure}{0.42\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Tps_Peer_bar.pdf}
		\caption{Average Tps with varying number of peers}
		\label{fig:tpspeer}
	\end{subfigure}
	\quad
	\begin{subfigure}{0.42\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Latency_Peer.pdf}
		\caption{Execution Time with varying number of peers}
		\label{fig:latencypeer}
	\end{subfigure}
	\caption{Performance and Scalability of Libra and Hyperledger Fabric}

\end{figure*}

